Photon-Photon Interactions in Dynamically Coupled Cavities

We study theoretically the interaction between two photons in a nonlinear cavity. The photons are loaded into the cavity via a method we propose here, in which the input/output coupling of the cavity is effectively controlled via a tunable coupling to a second cavity mode that is itself strongly output-coupled. Incoming photon wave packets can be loaded into the cavity with high fidelity when the timescale of the control is smaller than the duration of the wave packets. Dynamically coupled cavities can be used to avoid limitations in the photon-photon interaction time set by the delay-bandwidth product of passive cavities. Additionally, they enable the elimination of wave packet distortions caused by dispersive cavity transmission and reflection. We consider three kinds of nonlinearities, those arising from $\chi^{\scriptscriptstyle(2)}$ and $\chi^{\scriptscriptstyle(3)}$ materials and that due to an interaction with a two-level emitter. To analyze the input and output of few-photon wave packets we use a Schr\"odinger-picture formalism in which travelling-wave fields are discretized into infinitesimal time-bins. We suggest that dynamically coupled cavities provide a very useful tool for improving the performance of quantum devices relying on cavity-enhanced light-matter interactions such as single-photon sources and atom-like quantum memories with photon interfaces. As an example, we present simulation results showing that high fidelity two-qubit entangling gates may be constructed using any of the considered nonlinear interactions.

==> SPM.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Self Phase Modulation Analysis}\seclab{SPM eom}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Identical Input Photons V1}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
For identical input photons (the ideal case), the input state is
% 
\begin{align}
    \ket{\psi_0}=  \sqrt{2}\sum_{j=1}^N\sum_{k> j}^N \alpha_j \alpha_k  \Delta t \ket{00} \ket{ 1_j 1_k}, 
\end{align} 
%
After the first time step, the state is
% 
\begin{align}\eqlab{SPM photons step 1}  
    \ket{\psi_1} =  \hat{U}_1\ket{\psi_0} = \ket{\psi_0} +  \sqrt{2}\alpha_1\sqrt{\gamma}\Delta t \sum_{k>1}^N \alpha_k \sqrt{\Delta t} \ket{10}\ket{ 1_k} +\ldots ~\equiv
    \ket{\psi_0} +  \psi_{10}^{\rm{i}}(1)\!\sum_{k>1}^N \alpha_k \sqrt{\Delta t}\ket{10}\ket{1_k} +\ldots,
\end{align} 
%
where we defined the amplitude $\psi_{10}^{\rm{i}}(n)$ corresponding to one photon in mode $X$ at time $n$ with the other photon being on the input side. After step 2, this amplitude evolves as
% 
\begin{align}\eqlab{SPM 2 photons step 2 psi_10^i}  
    \ket{\psi_2} = \Big[\Big(1-\frac{\Gamma}{2}\Delta t - i2\mu|\kappa_2|\Delta t\Big)\psi_{10}^{\rm{i}}(1) + \sqrt{2}\alpha_2\sqrt{\gamma}\Delta t \Big]\psi_{10}^{\rm{i}}(1)\!\sum_{k>2}^N \alpha_k \sqrt{\Delta t} \ket{10}\ket{1_k} + \ldots
\end{align} 
%
The frequency conversion process generates states with one photon in mode $A$ and the other photon on the input side
% 
\begin{align}\eqlab{SPM 2 photons step 2 psi_01^i}  
    \ket{\psi_2} = -i\mu\kappa_2 \psi_{10}^{\rm{i}}(1)\!\sum_{k>2}^N \alpha_k \sqrt{\Delta t} \ket{01}\ket{1_k} + \ldots \equiv \psi_{01}^{\rm{i}}(2)\!\sum_{k>2}^N \alpha_k \sqrt{\Delta t} \ket{01}\ket{1_k} + \ldots 
\end{align} 
%
The photon from the input side may also be absorbed leading to a state with two photons in mode $X$
% 
\begin{align}\eqlab{SPM 2 photons step 2 psi_20}  
    \ket{\psi_2} &= \sqrt{2\gamma}\psi_{10}^{\rm{i}}(1) \Delta t \ket{20}\ket{\emptyset} + \ldots \equiv \psi_{20}(2) \Delta t \ket{20}\ket{\emptyset} + \ldots,
\end{align} 
%
where the factor of $\sqrt{2}$ comes from $\hat{a}_X^\dagger$ acting on $\ket{1_X}$. In the second step, the absorbed photon may be re-emitted 
% 
\begin{align}\eqlab{SPM 2 photons step 2 psi_00}  
    \ket{\psi_2} = - \sqrt{\gamma}\psi_{10}^{\rm{i}}(1)\sum_{k>2}^N  \alpha_k \Delta t  \ket{00} \ket{1_k \mathbf{1}_2}  + \ldots ,
    % \equiv \psi_{00}(2) \sum_{k>2}^N \Delta t  \ket{00} \ket{1_k \mathbf{1}_2},
\end{align} 
%
where boldface is used to indicate that the photon is on the output side.

All the dynamics necessary to determine equations of motion for $\psi_{10}^{\rm{i}}(t)$ and $\psi_{01}^{\rm{i}}(t)$ is present after step 3
% 
\begin{align}\eqlab{SPM 2 photons step 3 psi_10^i}  
    \ket{\psi_3} &=  \Big[\Big(1-\frac{\Gamma}{2}\Delta t - i2\mu|\kappa_3|\Delta t\Big)\psi_{10}^{\rm{i}}(2) + \sqrt{2}\alpha_3\sqrt{\gamma}\Delta t - i\mu\kappa_3^* \psi_{01}^{\rm{i}}(2)\Delta t \Big] \sum_{k>3}^N \!\alpha_k\sqrt{\Delta t} \ket{10}\ket{ 1_k}   +\ldots  \\
    \ket{\psi_3} &=  \Big[\big(1-\frac{\gamma_L}{2}\Delta t - i2\mu|\kappa_3|\Delta t\big)\psi_{01}^{\rm{i}}(2) - i\mu\kappa_3 \psi_{10}^{\rm{i}}(2) \Delta t\Big] \sum_{k>3}^N \!\alpha_k\sqrt{\Delta t} \ket{01}\ket{ 1_k}   + \ldots 
\end{align} 
%
In the continuum limit, this corresponds to a set of coupled ODEs
% 
\begin{align}\eqlab{SPM 2 photons ODE psi_10, psi_01} 
    \dot{\psi}_{10}^{\rm{i}}(t) &= -\Big(\frac{\Gamma}{2} + i2\mu|\kappa(t)|\Big)\psi_{10}^{\rm{i}}(t) - i\mu\kappa^{\!*}(t)\psi_{01}^{\rm{i}}(t) + \sqrt{2\gamma}\alpha(t) \\
    \dot{\psi}_{01}^{\rm{i}}(t) &= -\Big(\frac{\gamma_L}{2}+ i2\mu|\kappa(t)|\Big)\psi_{01}^{\rm{i}}(t) - i\mu\kappa(t)\psi_{10}^{\rm{i}}(t).
\end{align} 
%

Next, let us consider states with two photons in the system. Step 3 introduces the amplitude corresponding to one photon in each cavity mode
% 
\begin{align}\eqlab{SPM 2 photons step 3 psi_11}  
    \ket{\psi_3} &= \Big[\sqrt{\gamma} \psi_{01}^{\rm{i}}(2)\alpha_3 \Delta t - i \sqrt{2}\mu\kappa_3 \psi_{20}(2) \Delta t\Big] \ket{11}\ket{\emptyset}  + \ldots  \equiv \psi_{11}(3)\ket{11}\ket{\emptyset}  + \ldots
\end{align} 
%
Similarly, step 4 introduces the amplitude corresponding to both photons being in mode $A$
% 
\begin{align}\eqlab{SPM 2 photons step 3 psi_02}  
    \ket{\psi_4} &= -i\sqrt{2}\mu\kappa_4 \psi_{11}(3)\Delta t \ket{02}\ket{\emptyset}  + \ldots
\end{align} 
%
After step 5 all the dynamics describing the states with two photons in the system is present
% 
\begin{multline}\eqlab{2 cav modes 2 photons steps 3-5 two photon terms}
    \ket{\psi_5} = \Big[ \Big(1-\big(\Gamma+i\mu+i4\mu|\kappa_5|\big)\Delta t\Big)\psi_{20}(4)  -i\sqrt{2}\mu\kappa^*_5 \psi_{11}(4)\Delta t +  \psi_{10}(4)\alpha_5 \sqrt{2\gamma} \Delta t \Big] \ket{20}\ket{\emptyset} ~+\\
    \Big[ \Big(1 \minus \frac{\Gamma\plus\gamma_L}{2}\Delta t \minus \big(i\mu \plus  i4\mu|\kappa_5|\big)\Delta t \Big)\psi_{11}(4)  \minus i\sqrt{2}\mu\Delta t \big[ \kappa_5\psi_{20}(4) \plus \kappa_5^*\psi_{02}(4)\big] \plus \psi_{01}(4)\alpha_5\sqrt{\gamma}\Delta t \Big] \ket{11}\ket{\emptyset} +\\
    \Big[\Big(1-\big(\gamma_L+i\mu+i4\mu|\kappa_5|\big)\Delta t\Big)\psi_{02}(4) -i\sqrt{2}\mu\kappa_5 \psi_{11}(4) \Big]\!\ket{02}\!\ket{\emptyset} + \ldots
\end{multline}   
% 
We identify the equations of motion in the continuum limit
% 
\begin{subequations}
\begin{align}\eqlab{ODEs two photon terms} 
    \dot{\psi}_{20}(t)  &= -\big(\Gamma+i\mu +i4\mu|\kappa(t)|\big)\psi_{20}(t) - i\sqrt{2}\mu\kappa^{\!*}(t)\psi_{11}(t) + \sqrt{2\gamma}\psi_{10}(t)\alpha(t) \\
    \dot{\psi}_{11}(t)  &= -\Big(\frac{\Gamma+\gamma_L}{2}+i\mu+i4\mu|\kappa(t)|\Big)\psi_{11}(t) - i\sqrt{2}\mu\kappa(t)\psi_{20}(t) - i\sqrt{2}\mu\kappa^{\!*}(t)\psi_{02}(t) + \sqrt{\gamma}\psi_{01}(t)\alpha(t) \\
    \dot{\psi}_{02}(t)  &= -\big(\gamma_L+i\mu+i4\mu|\kappa(t)|\big)\psi_{02}(t) - i\sqrt{2}\mu\kappa(t)\psi_{11}(t) . 
\end{align}  
\end{subequations}
%
What remains is to consider the dynamics of states with one photon in the system at time $n$ while the other is on the output side in bin $k$ (where $k<n$ by the definition of the output side). There are four ways these states are created: 1) One of the photons from the state $\ket{20}$ is emitted into bin $k\equal n$. 2) The photon in mode $X$ is emitted from the state $\ket{11}$ into bin $k\equal n$. 3) States $\ket{10}$ or $\ket{01}$ exist at time $n$ while a photon in bin $k\equal n$ passes the system without interacting. 4) A photon is emitted from the state $\ket{10}$ into bin $k$ while the second photon is absorbed at time $n$. 
%
\begin{subequations}
\begin{align}
    1)~~&& \ket{\psi_n} &=  -\sqrt{2\gamma} \psi_{20}(n)\sqrt{\Delta t} \ket{10}\ket{\mathbf{1}_k} +\ldots  \equiv \psi_{10}^{\rm{o}}(k\equal n,n)\sqrt{\Delta t}\ket{10}\ket{\mathbf{1}_k} +\ldots \\
    2)~~&& \ket{\psi_n} &=  -\sqrt{\gamma} \psi_{11}(n)\sqrt{\Delta t} \ket{01}\ket{\mathbf{1}_k} +\ldots  \equiv \psi_{01}^{\rm{o}}(k\equal n,n)\sqrt{\Delta t}\ket{10}\ket{\mathbf{1}_k} +\ldots \\
    3)~~&& \ket{\psi_n} &=  \psi_{10}^{\rm{i}}(n)\alpha_k \sqrt{\Delta t} \ket{10}\ket{\mathbf{1}_k} +\ldots  \equiv \psi_{10}^{\rm{o}}(k\equal n,n)\sqrt{\Delta t}\ket{10}\ket{\mathbf{1}_k} +\ldots \\
    3)~~&& \ket{\psi_n} &=  \psi_{01}^{\rm{i}}(n)\alpha_k \sqrt{\Delta t} \ket{01}\ket{\mathbf{1}_k} +\ldots  \equiv \psi_{01}^{\rm{o}}(k\equal n,n)\sqrt{\Delta t}\ket{01}\ket{\mathbf{1}_k} +\ldots \\
    4)~~&& \ket{\psi_n} &=  -\gamma \psi_{10}^{\rm{i}}(k)\alpha_n\Delta t \sqrt{\Delta t} \ket{10}\ket{\mathbf{1}_k} +\ldots  \equiv \psi_{10}^{\rm{o}}(k,n)\sqrt{\Delta t}\ket{10}\ket{\mathbf{1}_k} +\ldots
\end{align} 
\end{subequations}
%
Once these states with an output photon in bin $k$ and a photon in the system at time $n>k$ exist, the dynamics of the corresponding amplitudes $\psi_{10}^{\rm{o}}(k,n)$ and $\psi_{01}^{\rm{o}}(k,n)$ is governed only by their mutual interaction 
% 
\begin{multline}\eqlab{SPM 2 photons psi_10^o} 
    \ket{\psi_n}  = \Big[ \Big(1-\frac{\Gamma}{2}\Delta t - i2\mu|\kappa_n|\Delta t\Big)\psi_{10}^{\rm{o}}(k,n) -i\mu\kappa_n^* \psi_{01}^{\rm{o}}(k,n)\Delta t \Big] \sqrt{\Delta t}\ket{10}\ket{\mathbf{1}_k} ~-\\
    \Big[ \Big(1-\frac{\gamma_L}{2}\Delta t - i2\mu|\kappa_n|\Delta t\Big)\psi_{01}^{\rm{o}}(k,n) -i\mu\kappa_n \psi_{10}^{\rm{o}}(k,n) \Delta t\Big] \sqrt{\Delta t}\ket{01}\ket{\mathbf{1}_k} + \ldots
\end{multline} 
% 
% The driving terms for $\psi_{10}^{\rm{o}}(k,n)$ correspond to a photon passing the system without interacting at time $k$ while the second photon is absorbed at time $n$, $\sqrt{2\gamma}\alpha_n\alpha_k$, and to an absorbed photon being emitted at time $k$ while the second photon is absorbed at time $n$, $-\gamma\psi_{10}^{\rm{i}}(k)\alpha_n$. 
Let us define functions $L_{10}(\tau,t)$, $L_{01}(\tau,t)$, $M_{10}(\tau,t)$, and $M_{10}(\tau,t)$ and write their equations of motion in the continuum limit according to~\eqref{SPM 2 photons psi_10^o}
% 
\begin{subequations}\eqlab{ODEs out L} 
\begin{align}
    \dot{L}_{10}(\tau,t) &= -\Big(\frac{\Gamma}{2} + i2\mu|\kappa(t)|\Big)L_{10}(\tau,t) - i\mu\kappa^{\!*}\!(t)L_{01}(\tau,t)  \\
    \dot{L}_{01}(\tau,t) &= -\Big(\frac{\gamma_L}{2} + i2\mu|\kappa(t)|\Big)L_{01}(\tau,t) - i\mu\kappa(t)L_{10}(\tau,t) ,
\end{align}  
\end{subequations}
% 
and  
\begin{subequations}\eqlab{ODEs out M} 
\begin{align}
    \dot{M}_{10}(\tau,t) &= -\Big(\frac{\Gamma}{2} + i2\mu|\kappa(t)|\Big)M_{10}(\tau,t) - i\mu\kappa^{\!*}\!(t)M_{01}(\tau,t)  \\
    \dot{M}_{01}(\tau,t) &= -\Big(\frac{\gamma_L}{2} + i2\mu|\kappa(t)|\Big)M_{01}(\tau,t) - i\mu\kappa(t)M_{10}(\tau,t) ,
\end{align}  
\end{subequations}
% 
where the initial conditions are: $L_{10}(\tau,\tau)\equal 1$, $L_{01}(\tau,\tau)\equal 0$, $M_{10}(\tau,\tau)\equal 0$, and $ M_{01}(\tau,\tau)\equal 1$ while $\tau\leq t$.

The output state is defined as 
% 
\begin{align}\eqlab{output def}
    \ket{\psi_{\rm{out}}} \equiv \int_0^T \!\!\!dt \! \int_0^T \!\!\!d\tau \xi_{\rm{out}}(\tau,t) \hat{b}_X^\dagger(\tau)\hat{b}_X^\dagger(t)  \ket{\emptyset}.
\end{align}
% 
There are several contributions to $\xi_{\rm{out}}(\tau, t)$, the first being from both photons passing the system without interacting
% 
\begin{align}\eqlab{xi out 0 absorbed}
    \xi_{\rm{out}}(\tau,t) = \alpha(\tau)\alpha(t) +\ldots
\end{align}
% 
There are also contributions from one photon being absorbed while the other is not
% 
\begin{align}\eqlab{xi out 1 absorbed}
    \xi_{\rm{out}}(\tau,t) = -\sqrt{\gamma}\psi_{10}^{\rm{i}}(\tau)\alpha(\tau) L_{10}(\tau, t) -\sqrt{\gamma}\psi_{01}^{\rm{i}}(\tau)\alpha(\tau) M_{10}(\tau, t)  - \gamma\psi_{10}^{\rm{i}}(\tau)\!\int_{\tau}^t \!\!\alpha(s) L_{10}(s,t) ds + \ldots
\end{align}
% 
The last term in~\eqref{xi out 1 absorbed} contains an integral because we must sum over all the bins between $\tau$ and $t$ where the second photon might be absorbed. Finally, there are contributions from both photons having been absorbed
% 
\begin{align}\eqlab{xi out 2 absorbed}
    \xi_{\rm{out}}(\tau,t) = \sqrt{2}\gamma\psi_{20}(\tau) L_{10}(\tau, t) +  \gamma\psi_{11}(\tau) M_{10}(\tau, t) + \ldots
\end{align}
% 
The output amplitude is therefore
% 
\begin{multline}\eqlab{xi out all}
    \xi_{\rm{out}}(\tau,t) = \alpha(\tau)\alpha(t) -\sqrt{\gamma}\psi_{10}^{\rm{i}}(\tau)\alpha(\tau) L_{10}(\tau, t) -\sqrt{\gamma}\psi_{01}^{\rm{i}}(\tau)\alpha(\tau) M_{10}(\tau, t) ~-\\
    \gamma\psi_{10}^{\rm{i}}(\tau)\!\int_{\tau}^t \!\!\alpha(s) L_{10}(s,t) ds + \sqrt{2}\gamma\psi_{20}(\tau) L_{10}(\tau, t) +  \gamma\psi_{11}(\tau) M_{10}(\tau, t) .
\end{multline}
% 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Identical Input Photons}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
For identical input photons (the ideal case), the input state is
% 
\begin{align}
    \ket{\psi_0}=  \sqrt{2}\sum_{j=1}^N\sum_{k>j}^N \alpha_j \alpha_k  \Delta t \ket{00} \ket{ 1_j 1_k}, 
\end{align} 
%
At time step $n$ it is useful to write the contribution from $\ket{\psi_0}$ as 
% 
\begin{align}\eqlab{SPM photons step 0 at n}
    \ket{\psi_0(n)}=  \sqrt{2}\sum_{j=n}^N\sum_{k>j}^N \alpha_j \alpha_k  \Delta t \ket{00} \ket{ 1_j 1_k} + \sqrt{2}\sum_{j=1}^n\sum_{k>j}^n \alpha_j \alpha_k  \Delta t \ket{00} \ket{ \mathbf{1}_j \mathbf{1}_k} + \sqrt{2}\sum_{j=1}^n\sum_{k>n}^N \alpha_j \alpha_k  \Delta t \ket{00} \ket{ \mathbf{1}_j 1_k}. 
\end{align} 
%
The first term corresponds to both photons being on the input side. The second term corresponds to both photons having passed by the system without interacting and now being on the output side. The last term corresponds to one photon having passed by the system without interacting and the other photon remaining on the input side. Note that we use boldface to indicate photons on the output side.
After the first time step, the state is
% 
\begin{align}\eqlab{SPM photons step 1}  
    \ket{\psi_1} =  \hat{U}_1\ket{\psi_0} = \ket{\psi_0} +  \sqrt{2}\alpha_1\sqrt{\gamma}\Delta t \sum_{k=1}^N \alpha_k \sqrt{\Delta t} \ket{10}\ket{ 1_k} ~\equiv
    \ket{\psi_0} +  \!\sum_{k=1}^N \psi_{10}(k,1) \sqrt{\Delta t}\ket{10}\ket{1_k} .
\end{align} 
%
The amplitude $\psi_{10}(k,n)$ corresponds to one photon occupying mode $X$ at time step $n$ while the other photon is in the waveguide in bin $k$. Note that bins $k>n$ are on the input side while bins $k<n$ are on the output side.
In the second step, the absorbed photon may be re-emitted 
% 
\begin{align}\eqlab{SPM 2 photons step 2 psi_00}  
    \ket{\psi_2} = - \sqrt{\gamma}\sum_{k=1}^N \psi_{10}(k,1) \Delta t  \ket{00} \ket{1_k 1_2}  + \ldots \equiv \sum_{k=1}^N \psi_{00}(k,2)\Delta t  \ket{00} \ket{1_k 1_2}.
\end{align} 
%
Updating $\psi_{10}$ requires splitting the summation into $k<n$ and $k>n$ because different processes are possible depending on whether the waveguide photon is on the input or output side. For both cases, the photon in mode $X$ may decay or undergo cross phase modulation due to the pump fields. For $k>n$, the waveguide photon may also be absorbed. We therefore have
% 
\begin{subequations}\eqlab{SPM 2 photons step 2 psi_10}  
\begin{align}
    \ket{\psi_2} &= \Big(1-\frac{\Gamma}{2}\Delta t - i2\mu|\kappa_2|\Delta t\Big)\psi_{10}(1,1)  \sqrt{\Delta t} \ket{10}\ket{1_1} +\ldots \equiv \psi_{10}(1,2) \sqrt{\Delta t} \ket{10}\ket{1_1} +\ldots \\
    \ket{\psi_2} &= \sum_{k=2}^N \Big[\big(1-\frac{\Gamma}{2}\Delta t - i2\mu|\kappa_2|\Delta t\big)\psi_{10}(k,1) + \sqrt{2}\alpha_2\alpha_k\sqrt{\gamma}\Delta t \Big]\sqrt{\Delta t} \ket{10}\ket{1_k} + \ldots 
    % \equiv \sum_{k=2}^N \psi_{10}(k,2) \sqrt{\Delta t} \ket{10}\ket{1_k} +\ldots 
\end{align} 
\end{subequations}
%
Another process that can occur in step 2 is for the photon in mode $X$ to be converted to mode $A$ 
% 
\begin{align}\eqlab{SPM 2 photons step 2 psi_01}  
    \ket{\psi_2} &= \sum_{k=1}^N -i\mu\kappa_2\Delta t \psi_{10}(k,1) \sqrt{\Delta t} \ket{01}\ket{1_k} + \ldots
\end{align} 
%
Additionally, if the waveguide photon is on the input side, it may be absorbed into mode $X$
% 
\begin{align}\eqlab{SPM 2 photons step 2 psi_20}  
    \ket{\psi_2} &= \sqrt{2\gamma}\psi_{10}(2,1) \Delta t \ket{20}\ket{\emptyset} + \ldots \equiv \psi_{20}(2) \Delta t \ket{20}\ket{\emptyset} + \ldots,
\end{align} 
%
where the factor of $\sqrt{2}$ comes from $\hat{a}_X^\dagger$ acting on $\ket{1_X}$.

In step 3, new terms appear in the dynamics of $\psi_{10}$ due to BS-FWM as well as driving by $\psi_{00}$ and $\psi_{20}$
% 
\begin{subequations}\eqlab{SPM 2 photons step 3 psi_10}  
\begin{align}
    \ket{\psi_3} &= \Big[\Big(1-\frac{\Gamma}{2}\Delta t - i2\mu|\kappa_3|\Delta t\Big)\psi_{10}(1,2) -i\mu\kappa_3^*\psi_{01}(1,2) \Big] \sqrt{\Delta t} \ket{10}\ket{1_1} +\ldots\\
    \ket{\psi_3} &= \Big[\Big(1-\frac{\Gamma}{2}\Delta t - i2\mu|\kappa_3|\Delta t\Big)\psi_{10}(2,2)  + \Big(\sqrt{\gamma}\psi_{00}(3,2) -i\mu\kappa_3^*\psi_{01}(2,2)\Big)\Delta t \Big] \sqrt{\Delta t} \ket{10}\ket{1_2} +\ldots\\
    % \ket{\psi_3} &= \Big(1-\frac{\Gamma}{2}\Delta t - i2\mu|\kappa_3|\Delta t\Big)\psi_{10}(k,2)  \sqrt{\Delta t} \ket{10}\ket{1_2} +\ldots\\
    \ket{\psi_3} &= \Big[\big(1-\frac{\Gamma}{2}\Delta t - i2\mu|\kappa_3|\Delta t\big)\psi_{10}(3,2)  + \Big(\sqrt{2}\alpha_3\alpha_3\sqrt{\gamma} -i\mu\kappa_3^*\psi_{01}(3,2) -\sqrt{2\gamma}\psi_{20}(2)\Big)\Delta t\Big]\sqrt{\Delta t} \ket{10}\ket{1_3} + \ldots \\
    \ket{\psi_3} &= \sum_{k=4}^N \Big[\big(1-\frac{\Gamma}{2}\Delta t - i2\mu|\kappa_3|\Delta t\big)\psi_{10}(k,2)  + \Big(\sqrt{2}\alpha_3\alpha_k\sqrt{\gamma}-i\mu\kappa_3^*\psi_{01}(k,2)\Big)\Delta t \Big]\sqrt{\Delta t} \ket{10}\ket{1_k} + \ldots
\end{align} 
\end{subequations}
%
The dynamics for $\psi_{20}$ is 
% 
\begin{align}\eqlab{SPM 2 photons step 3 psi_20}  
    \ket{\psi_3} &= \Big[\big( 1 - \Gamma\Delta t - i4\mu|\kappa_3| \big)\psi_{20}(2) + \sqrt{2\gamma}\psi_{10}(3,2) \Delta t \Big] \ket{20}\ket{\emptyset}  + \ldots  
\end{align} 
%
Step 3 also introduces the state $\ket{11}$, which is driven by absorption of a photon while mode $A$ is occupied (corresponding to $\psi_{01}$) or frequency conversion of one of the photons in mode $X$ (from $\psi_{20}$)
% 
\begin{align}\eqlab{SPM 2 photons step 3 psi_11}  
    \ket{\psi_3} &= \Big[\sqrt{\gamma} \psi_{01}(3,2)\Delta t - i \sqrt{2}\mu\kappa_3 \psi_{20}(2) \Delta t\Big] \ket{11}\ket{\emptyset}  + \ldots  \equiv \psi_{11}(3)\ket{11}\ket{\emptyset}  + \ldots
\end{align} 
%
Let us go to step 4 to introduce the last type of state, $\ket{02}$, which originates in conversion from mode $X$ to mode $A$ when the state is $\ket{11}$
% 
\begin{align}\eqlab{SPM 2 photons step 2 psi_02}  
    \ket{\psi_4} &= - i \sqrt{2}\mu\kappa_4 \psi_{11}(3) \Delta t \ket{02}\ket{\emptyset}  + \ldots  \equiv \psi_{02}(4)\ket{02}\ket{\emptyset}  + \ldots
\end{align} 
%
Moving to step 5 allows us to write out all the possible dynamics. First, we consider state $\ket{10}$
% 
\begin{subequations}\eqlab{SPM 2 photons step 5 psi_10}  
\begin{align}
    % \ket{\psi_5} &= \Big[\Big(1-\frac{\Gamma}{2}\Delta t - i2\mu|\kappa_5|\Delta t\Big)\psi_{10}(1,4) -i\mu\kappa_5^*\psi_{01}(1,4) \Big] \sqrt{\Delta t} \ket{10}\ket{1_1} +\ldots\\
    \ket{\psi_5} &= \!\sum_{k=1}^4\Big[\Big(1-\frac{\Gamma}{2}\Delta t - i2\mu|\kappa_5|\Delta t\Big)\psi_{10}(k,4)  + \Big(\sqrt{\gamma}\psi_{00}(5,k) -i\mu\kappa_5^*\psi_{01}(k,4) \Big)\Delta t  \Big] \sqrt{\Delta t} \ket{10}\ket{1_k} +\ldots\\
    % \ket{\psi_5} &= \Big[\Big(1-\frac{\Gamma}{2}\Delta t - i2\mu|\kappa_5|\Delta t\Big)\psi_{10}(3,4) -i\mu\kappa_5^*\psi_{01}(3,4) + \sqrt{\gamma}\psi_{00}(5,3)\Delta t  \Big] \sqrt{\Delta t} \ket{10}\ket{1_3} +\ldots\\
    % \ket{\psi_3} &= \Big(1-\frac{\Gamma}{2}\Delta t - i2\mu|\kappa_3|\Delta t\Big)\psi_{10}(k,2)  \sqrt{\Delta t} \ket{10}\ket{1_2} +\ldots\\
    \ket{\psi_5} &= \!\Big[\big(1-\frac{\Gamma}{2}\Delta t - i2\mu|\kappa_5|\Delta t\big)\psi_{10}(5,4)  + \Big(\sqrt{2}\alpha_5\alpha_5\sqrt{\gamma}-i\mu\kappa_5^*\psi_{01}(5,4) -\sqrt{2\gamma}\psi_{20}(4)\Big)\Delta t\Big]\sqrt{\Delta t} \ket{10}\ket{1_5} + \ldots \\
    \ket{\psi_5} &= \!\sum_{k=6}^N \Big[\big(1-\frac{\Gamma}{2}\Delta t - i2\mu|\kappa_5|\Delta t\big)\psi_{10}(k,4)  + \Big(\sqrt{2}\alpha_5\alpha_k\sqrt{\gamma}-i\mu\kappa_5^*\psi_{01}(k,4)\Big) \Delta t \Big]\sqrt{\Delta t} \ket{10}\ket{1_k} + \ldots
\end{align} 
\end{subequations}
%
Next, we consider $\ket{01}$
% 
\begin{subequations}\eqlab{SPM 2 photons step 5 psi_01}  
\begin{align}
    % \ket{\psi_5} &= \Big[\Big(1-\frac{\Gamma}{2}\Delta t - i2\mu|\kappa_5|\Delta t\Big)\psi_{10}(1,4) -i\mu\kappa_5^*\psi_{01}(1,4) \Big] \sqrt{\Delta t} \ket{10}\ket{1_1} +\ldots\\
    \ket{\psi_5} &= \!\sum_{k=1}^4\Big[\Big(1-\frac{\gamma_L}{2}\Delta t - i2\mu|\kappa_5|\Delta t\Big)\psi_{01}(k,4) -i\mu\kappa_5\psi_{10}(k,4)\Delta t   \Big] \sqrt{\Delta t} \ket{01}\ket{1_k} +\ldots\\
    % \ket{\psi_5} &= \Big[\Big(1-\frac{\Gamma}{2}\Delta t - i2\mu|\kappa_5|\Delta t\Big)\psi_{10}(3,4) -i\mu\kappa_5^*\psi_{01}(3,4) + \sqrt{\gamma}\psi_{00}(5,3)\Delta t  \Big] \sqrt{\Delta t} \ket{10}\ket{1_3} +\ldots\\
    % \ket{\psi_3} &= \Big(1-\frac{\Gamma}{2}\Delta t - i2\mu|\kappa_3|\Delta t\Big)\psi_{10}(k,2)  \sqrt{\Delta t} \ket{10}\ket{1_2} +\ldots\\
    \ket{\psi_5} &= \!\Big[\big(1-\frac{\Gamma}{2}\Delta t - i2\mu|\kappa_5|\Delta t\big)\psi_{01}(5,4) -\Big(i\mu\kappa_5\psi_{10}(5,4) - \sqrt{\gamma}\psi_{11}(4)\Big)\Delta t\Big]\sqrt{\Delta t} \ket{10}\ket{1_5} + \ldots \\
    \ket{\psi_5} &= \!\sum_{k=6}^N \Big[\big(1-\frac{\Gamma}{2}\Delta t - i2\mu|\kappa_5|\Delta t\big)\psi_{10}(k,4)  + \Big(\sqrt{2}\alpha_5\alpha_k\sqrt{\gamma}-i\mu\kappa_5^*\psi_{01}(k,4)\Big)\Delta t \Big]\sqrt{\Delta t} \ket{10}\ket{1_k} + \ldots
\end{align} 
\end{subequations}
%
rrl\\
% 
\begin{subequations}\eqlab{SPM 2 photons psi_10}  
\begin{align}
    \frac{d}{dt}\Big(\psi_{10}(\tau, t)\Big) &= \Big(-\frac{\Gamma}{2} - i2\mu|\kappa_5| t\Big)\psi_{10}(\tau,t) -\gamma\psi_{10}(t,\tau) -i\mu\kappa^{\!*}(t)\psi_{01}(\tau, t) , ~\tau<t \\
    % \ket{\psi_5} &= \!\Big[\big(1-\frac{\Gamma}{2}\Delta t - i2\mu|\kappa_5|\Delta t\big)\psi_{10}(5,4)  + \Big(\sqrt{2}\alpha_5\alpha_5\sqrt{\gamma}-i\mu\kappa_5^*\psi_{01}(5,4) -\sqrt{2\gamma}\psi_{20}(4)\Big)\Delta t\Big]\sqrt{\Delta t} \ket{10}\ket{1_5} + \ldots \\
    % \ket{\psi_5} &= \!\sum_{k=6}^N \Big[\big(1-\frac{\Gamma}{2}\Delta t - i2\mu|\kappa_5|\Delta t\big)\psi_{10}(k,4)  + \Big(\sqrt{2}\alpha_5\alpha_k\sqrt{\gamma}-i\mu\kappa_5^*\psi_{01}(k,4)\Big) \Delta t \Big]\sqrt{\Delta t} \ket{10}\ket{1_k} + \ldots
\end{align} 
\end{subequations}
%




The amplitude $\psi_{10}^{\rm{o}}(m,n)$ corresponds to a photon passing the system without interaction in bin $m$ while the second photon is in mode $X$ in bin $n$. 

In the second step, the absorbed photon may be re-emitted 
% 
\begin{align}\eqlab{SPM 2 photons step 2 psi_00}  
    \ket{\psi_2} = - \sqrt{\gamma}\psi_{10}^{\rm{i}}(1)\alpha_2 \Delta t  \ket{00}\!\ket{\mathbf{1}_2 \mathbf{1}_2} - \sqrt{\gamma}\psi_{10}^{\rm{i}}(1) \!\sum_{k>2}^N \alpha_k \Delta t  \ket{00}\!\ket{\mathbf{1}_2 1_k} - \sqrt{\gamma}\psi_{10}^{\rm{o}}(1,1)\Delta t\ket{00}\!\ket{\mathbf{1}_1\mathbf{1}_2}  + \ldots 
    % ~\equiv \psi_{00}(2,2)\!\sum_{k>2}^N \alpha_k \Delta t  \ket{00}\!\ket{\mathbf{1}_2 1_k} + \ldots 
\end{align} 
%
The first term corresponds to $(k\equal 2)$ in the summation of the second term. The reason for pulling it out of the summation is that bin 2 changes from input to output in step 2, so $k$ must start at 3 in the summation in order for $\psi_{10}^{\rm{i}}$ to correspond to a photon in mode $X$ and a photon on the input side. The first and last terms in~\eqref{SPM 2 photons step 2 psi_00} contribute to the output wave packet since both photons are on the output side.

Let us follow states with one photon in mode $X$ after step 2
% 
\begin{multline}\eqlab{SPM 2 photons step 2 psi_10^i}  
    \ket{\psi_2} = \Big[\big(1-\frac{\Gamma}{2}\Delta t - i2\mu|\kappa_2|\Delta t\big)\psi_{10}^{\rm{i}}(1) + \sqrt{2}\alpha_2\sqrt{\gamma}\Delta t \Big]\psi_{10}^{\rm{i}}(1)\!\sum_{k>2}^N \alpha_k \sqrt{\Delta t} \ket{10}\!\ket{1_k} ~+\\
    \Big[\psi_{10}^{\rm{i}}(2)\alpha_2 + \sqrt{2}\alpha_2\alpha_2 \sqrt{\gamma} \Delta t \Big] \sqrt{\Delta t} \ket{10}\!\ket{\mathbf{1}_2} + \ldots
\end{multline} 
%
ehr\\

Note that the summation over $k$ now starts at 3. The term with $k\equal 2$ now corresponds to a state with two photons on the output because each time step adds another bin to the output side and subtracts one from the input side, see~\figref{discrete time illustration}. This term adds a contribution to the output wave packet 
% 
\begin{align}\eqlab{SPM 2 photons alpha out phi_10^i}  
    \ket{\psi_2} = - \sqrt{\gamma}\psi_{10}^{\rm{i}}(1)\alpha_2 \ket{00}\!\ket{\mathbf{1}_2 \mathbf{1}_2} + \ldots \equiv \alpha_{\rm{out}}(2,2) \ket{00}\!\ket{\mathbf{1}_2 \mathbf{1}_2} + \ldots
\end{align} 
%
Another contribution to the state at time step 2 comes from the input photon in the last term of~\eqref{SPM photons step 0 at n} being absorbed
% 
\begin{align}\eqlab{SPM 2 photons step 2 psi_10^o}  
    \ket{\psi_2} &=  \sqrt{2}\alpha_2 \Delta t \sqrt{\Delta t}\ket{10}\!\ket{\mathbf{1}_1}   + \ldots \equiv + \psi_{10}^{\rm{o}}(1, 2) \sqrt{\Delta t}\ket{10}\!\ket{\mathbf{1}_1}   + \ldots
\end{align} 
%
The remaining contributions to the state at step 2 correspond to the second photon being absorbed into mode $X$
% 
\begin{align}\eqlab{SPM 2 photons step 2 psi_20}  
    \ket{\psi_2} &=  \sqrt{2\gamma} \psi_{10}^{\rm{i}}(1)\alpha_2  \Delta t\ket{20}\!\ket{\emptyset}   + \ldots \equiv \psi_{20}(2)\ket{20}\!\ket{\emptyset} ,
\end{align} 
%
and the first absorbed photon being converted to mode $A$ 
% 
\begin{align}\eqlab{SPM 2 photons step 2 psi_01^i}  
    \ket{\psi_2} &=  -i\mu \kappa_2 \psi_{10}^{\rm{i}}(1) \Delta t\!\sum_{k>2}^N \alpha_k \sqrt{\Delta t}  \ket{01}\!\ket{1_k}  + \ldots \equiv \psi_{01}^{\rm{i}}(2)\!\sum_{k>2}^N \alpha_k \sqrt{\Delta t} \ket{01}\!\ket{1_k}  + \ldots  
\end{align} 
%
Step 2 modifies the state with one photon in mode $X$ and one photon on the input side as
% 
\begin{align}\eqlab{SPM 2 photons step 2 psi_10^i}  
    \ket{\psi_2} &=  \Big[\big(1-\frac{\Gamma}{2}\Delta t - i2\mu|\kappa_2|\Delta t\big)\psi_{10}^{\rm{i}}(1) + \sqrt{2}\alpha_2\sqrt{\gamma}\Delta t \Big] \sum_{k>2}^N \!\alpha_k\sqrt{\Delta t} \!\ket{10}\!\ket{ 1_k}   + \ldots  \equiv \psi_{10}^{\rm{i}}(2)\sum_{k>2}^N \!\alpha_k\sqrt{\Delta t} \!\ket{10}\!\ket{ 1_k} .
\end{align} 
%
All the dynamics necessary to determine equations of motion for $\psi_{10}^{\rm{i}}(t)$ and $\psi_{01}^{\rm{i}}(t)$ are present after step 3
% 
\begin{align}\eqlab{SPM 2 photons step 3 psi_10^i}  
    \ket{\psi_3} &=  \Big[\Big(1-\frac{\Gamma}{2}\Delta t - i2\mu|\kappa_3|\Delta t\Big)\psi_{10}^{\rm{i}}(2) + \sqrt{2}\alpha_3\sqrt{\gamma}\Delta t - i\mu\kappa_3^* \psi_{01}^{\rm{i}}(2)\Delta t \Big] \sum_{k>3}^N \!\alpha_k\sqrt{\Delta t} \!\ket{10}\!\ket{ 1_k}   +\ldots  \\
    \ket{\psi_3} &=  \Big[\big(1-\frac{\gamma_L}{2}\Delta t - i2\mu|\kappa_3|\Delta t\big)\psi_{01}^{\rm{i}}(2) - i\mu\kappa_3 \psi_{10}^{\rm{i}}(2) \Delta t\Big] \sum_{k>3}^N \!\alpha_k\sqrt{\Delta t} \!\ket{01}\!\ket{ 1_k}   + \ldots 
\end{align} 
%
In the continuum limit, this corresponds to a set of coupled ODEs
% 
\begin{align}\eqlab{SPM 2 photons ODE psi_10, psi_01} 
    \dot{\psi}_{10}^{\rm{i}}(t) &= -\Big(\frac{\Gamma}{2} + i2\mu|\kappa(t)|\Big)\psi_{10}^{\rm{i}}(t) - i\mu\kappa^{\!*}(t)\psi_{01}^{\rm{i}}(t) + \sqrt{2\gamma}\alpha(t) \\
    \dot{\psi}_{01}^{\rm{i}}(t) &= -\Big(\frac{\gamma_L}{2}+ i2\mu|\kappa(t)|\Big)\psi_{01}^{\rm{i}}(t) - i\mu\kappa(t)\psi_{10}^{\rm{i}}(t).
\end{align} 
%
Let us follow the evolution of states with oe photon in mode $A$ and one photon on the output side
% 
\begin{align}\eqlab{SPM 2 photons step 3 psi_10^o}  
    \ket{\psi_3} &= \Big[\Big(1-\frac{\Gamma}{2}\Delta t - i2\mu|\kappa_3|\Delta t\Big)\psi_{10}^{\rm{o}}(1,2) \Big] \sqrt{\Delta t}\ket{10}\!\ket{\mathbf{1}_1} + \sqrt{2}\alpha_3 \Delta t \sqrt{\Delta t}\ket{10}\!\ket{\mathbf{1}_1}   + \ldots \equiv + \psi_{10}^{\rm{o}}(1, 2) \sqrt{\Delta t}\ket{10}\!\ket{\mathbf{1}_1}   + \ldots
\end{align} 
%



Step 3 also introduces a new type of state. A photon from the input side may be absorbed while the other photon is in mode $A$ or one of the photons in mode $X$ may be converted to mode $A$
% 
\begin{align}\eqlab{SPM 2 photons step 3 psi_11}  
    \ket{\psi_3} &= \Big[\sqrt{\gamma} \psi_{01}^{\rm{i}}(2)\alpha_3 \Delta t - i \sqrt{2}\mu\kappa_3 \psi_{20}(2) \Delta t\Big] \!\ket{11}\!\ket{\emptyset}  + \ldots  \equiv \psi_{11}(3)\!\ket{11}\!\ket{\emptyset}  + \ldots
\end{align} 
%


==> app_nonlinear_coupling_coefficients.tex <==






\section{Nonlinear Coupling Rates \applab{nonlinear coupling rates}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this section we relate the nonlinear coupling rates in the Hamiltonian to measurable material parameters.
The displacement field is
% 
\begin{align}\eqlab{D field}
    \hat{\bm{D}}(\bm{r},t) &= \sum_\nu \int_\beta d\beta \Big( \hat{\bm{D}}_{\nu \beta}(\bm{r}) e^{-i\omega_{\nu \beta} t} + \hat{\bm{D}}_{\nu \beta}^\dagger(\bm{r}) e^{i\omega_{\nu \beta} t} \Big) \\
    \hat{\bm{D}}_{\nu \beta}(\bm{r}) &= \sqrt{\frac{\hbar \omega_{\nu \beta}}{2}} \hat{a}_{\nu \beta} \bm{d}_{\nu \beta}(\bm{r}), 
\end{align} 
%
where $\bm{d}_{\nu \beta}(\bm{r})$ describes the electromagnetic field profile of mode $\nu$ with wave number $\beta$ found by solving Maxwell's equations. [how is it normalized?].\\

The constitutive relation is
% 
\begin{align}\eqlab{P field}
    \bm{D}(\bm{r},t) &= \epsilon_0 \bm{E}(\bm{r},t) +  \bm{P}(\bm{r},t) \\
    P_i(\bm{r},t) &= \sum_j \Gamma_{ij}^{(1)} D_j(\bm{r},t) + \sum_{jk} \Gamma_{ijk}^{(2)} D_j(\bm{r},t)D_k(\bm{r},t) + \sum_{jkl} \Gamma_{ijkl}^{(3)} D_j(\bm{r},t)D_k(\bm{r},t)D_l(\bm{r},t) + \ldots 
\end{align} 
%

We consider cavity modes and drop the integration over $k$.\\
The nonlinear Hamiltonian is~\cite{Sipe2004}
% 
\begin{align}\eqlab{HNL D field}
    \hat{H}_{\!N\!L} = -\frac{1}{3\epsilon_0} \int d\bm{r} \Gamma^{(2)}(\bm{r}) \hat{\bm{D}}^3(\bm{r})  -\frac{1}{4\epsilon_0} \int d\bm{r} \Gamma^{(3)}(\bm{r}) \hat{\bm{D}}^4(\bm{r}) .
\end{align} 
%

% 
\begin{align}\eqlab{H_SHG D field}
    \hat{H}_{\!S\!H\!G} = -\frac{1}{3\epsilon_0}\Big(\frac{3!}{2!1!}\Big) \sqrt{\frac{\hbar^3 \omega_{\nu}^2\omega_\mu}{8}}\bigg[ \hat{a}_\nu\hat{a}_\nu\hat{a}_\mu^\dagger \int d\bm{r} \Gamma^{(2)} (\bm{r}) d_{\nu}(\bm{r}) d_{\nu }(\bm{r}) d_{\mu}^*(\bm{r})   + \hat{a}_\nu^\dagger\hat{a}_\nu^\dagger\hat{a}_\mu \int d\bm{r} \Gamma^{(2)} (\bm{r}) d_{\nu}^*(\bm{r}) d_{\nu }^*(\bm{r}) d_{\mu}(\bm{r})\bigg]
\end{align} 
%


\subsection{$\chi^{(3)}$ material}
% 
\begin{align}\eqlab{chi3 nonlinear coupling rate}
    \chi_3 = \frac{2\hbar\overline{\omega}^2 c n_2}{\overline{n}^2 V_{\rm{mode}}}
\end{align} 
%

==> app_nonlinear_dynamics.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Nonlinear Dynamics \applab{nonlinear dynamics}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The nonlinear unitary is
% 
\begin{multline}
    \hat{U}_n^{\rm{lin},\chi^{\scriptscriptstyle \!(3)}} \!\!= \hat{\mathbb{I}} + \sqrt{\gamma \Delta t} \Big(\hat{a}^\dagger \hat{w}_n \minus \hat{a} \hat{w}_n^\dagger  \Big) - \frac{\gamma}{2}\Delta t \hat{a}^\dagger \hat{a} \hat{w}_n\hat{w}_n^\dagger  ~-\\
    i\Delta t\mu \Big(\kappa_n^* \hat{a}^\dagger\hat{b} + \kappa_n\hat{b}^\dagger\hat{a}\Big) -i2\mu |\kappa_n| \Big(\hat{b}^\dagger\hat{b} \plus \hat{a}^\dagger\hat{a} \Big) ~-\\
    i\Delta t\mu \hat{b}^\dagger\hat{b}\hat{a}^\dagger\hat{a} - i\frac12 \Delta t \mu \Big[ \big( \hat{b}^\dagger\hat{b}\minus1\big)\hat{b}^\dagger\hat{b} + \big( \hat{a}^\dagger\hat{a}\minus1\big)\hat{a}^\dagger\hat{a} \Big].
\end{multline} 
% 

==> couped_resonators_mode_analysis.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Mode Structure of Coupled Ring Resonators}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{align}\eqlab{circ field}
I_{\rm{circ}}/I_0 = \frac{1}{1 - C_{11}^{(1)}e^{i\Phi_1} t_2 t_3},  
\end{align}
%
where $t_{2/3}$ is 
%
\begin{align}\eqlab{t 2/3}
t_{2/3} = C_{11}^{(2/3)} + \frac{C_{12}^{(2/3)}C_{21}^{(2/3)}e^{i\Phi_{2/3}}}{1 - C_{22}^{(2/3)}e^{i\Phi_{2/3}}},  
\end{align}
%
with the coupling matrices given by 
%
\begin{align}\eqlab{C 2/3}
\bm{C}^{(1)} \!&= \!\!\left[\!\!\begin{array}{c c} \eta_1^2 \minus e^{i\psi}( 1 \minus \eta_1^2) 	& \!\!i\eta_1\sqrt{1\minus\eta_1^2} \big(1\plus e^{i\psi}\big) \\
i\eta_1\sqrt{1\minus\eta_1^2} \big(1\plus e^{i\psi}\big)  	& \!\!\eta_1^2\big(1\plus e^{i\psi}\big) \minus 1  \end{array} \!\!\right] \\
\bm{C}^{(2/3)} \!&= \!\!\left[\!\!\begin{array}{c c} \eta_{2/3}	& i\sqrt{1\minus \eta_{2/3}^2} \\
i\sqrt{1\minus \eta_{2/3}^2} 	& \eta_{2/3}  \end{array} \right]
\end{align} 



% \section{\label{sec:intro}Introduction}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Implementation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The structure is illustrated in~\figref{XPM sketch} and consists of three rings with circumferences $L_2\equal L_1/6$ and $L_3\equal L_1/12$. A Mach-Zehnder Interferometer (MZI) with a path-length difference, $L_{\psi}\equal L_1/6$, is formed between ring 1 and the waveguide giving rise to interferometric coupling~\cite{Madsen1999}.
%
\begin{figure}[htb]   %generated by 
\centering
   \includegraphics[width=8.4cm] {./XPM_PIC_concept.pdf}
\caption{Sketch of resonator architecture for loading and unloading via BS-FWM.  }
\figlab{XPM sketch}
\end{figure} 
%


==> kurt_derivation.tex <==
\section{Equations of motion for the Cross-Kerr Gate}

In Section~\ref{***} we derived the equations of motion for two cavity modes, in which one had a single photon input, and was coupled to a second cavity via a controllable coupling. This coupling was used to load the second cavity via the first. Now we need to derive the equations of motion of two such twin-cavity systems, where there is a cross-Kerr interaction between the two cavities that get loaded, each with a single photon. 

A direct derivation of this four-cavity system, the approach we took for deriving the twin-cavity system, is very complex. One can get a long way in deriving these equations by first moting that appart from the cross-Kerr Hamiltonian the evoution of the two twin-cavity systems is merely that of the tensor product of the two independent evolutions. Adding the cross-Kerr term can then be done fairly intuitively. Neverthless one would like a more systematic way to derive the equations. 

We will take a two-stage approach here. First we will examine the structure of the evolution of just two cavities in which each has its own single-photon input. This is the evolution of the auiliary cavities without their coupling to the cavities that get loaded with the single photons. This analysis will give us insight into the form that the equations take, and how the output field, which is now a joint field of two photons, one in each output channel,  can be written directly in terms of the states of the cavity modes, generalizing the result for a single mode in Eq.(\ref{***}). This will allow us to write down the equations of motion for the two auxiliary cavities, and including the coherent coupling to the two primary cavities is fairly straightforward. However, since the above method is not systematic, it leaves open the possibility that we may have left something out. To address this will then apply the Hamiltonian of the full four-cavity system to the initial state, for delta-function input envelopes, to propagate it a number of time-steps. This generates the entire structure of the evolution, and allows us to directly verify the equations of motion that we have derived. 

\subsection{Analyzing the structure of the dynamics for two separate cavities}

Let us first briefly review the  Schr\"{o}dinger picture version of input-output theory for single-photon input. Discretizing the input field into chunks of time $\Delta t$, something that has been called the ``collision model'' of open systems, gives the discretized input field operators  
\begin{align}
   b_{\mbox{\scriptsize in}}(t_j) =  b_{\mbox{\scriptsize in}}(j \Delta t) = \frac{b_j}{\sqrt{\Delta t}}  \;\;\; \mbox{with} \;\;\;  [b_j,b_k^\dagger] = \delta_{jk} ,  
\end{align}
These are the usual single mode creation and annihilation operators but with a factor of $1/\sqrt{\Delta t}$ that allows them to have the delta commutation relations as $\Delta t \rightarrow 0$. This formulation is nice because we see how the $\sqrt{\Delta t}$ is required to describe the effective "white noise" input of the vacuum field. 

Each of our two systems is coupled to a single input field with a single-photon input envelope. Each input field is a long sequence of time bins, labelled by $j$. At each time, the system interacts with only one bin in each input field, so this makes the dynamics rather different from the usual evolution of a closed system. In fact it simplifies the evolution a great deal as far as the field is concerned. The state of each input field is a single photon envelope 
\begin{align}
   |\psi_b\rangle = \sum_{j} \alpha_j \Delta t b_{\mbox{\scriptsize in}}^\dagger(j \Delta t) |0\rangle = \sum_{j} \sqrt{\Delta t} \alpha_j  b_j^\dagger |0\rangle . 
\end{align}
Thus the field state is a superposition of field states that each have a photon in only one bin, and each in a different bin. Thus when the system interacts with bin $j$ it can only absorb a photon from the single state that has a photon in that bin. 

\subsubsection{Revisiting a single mode with a single-photon input}

First we will revisit the derivation of the equations of motion for a single cavity interacting with a single input/output field. The system can contain at most one photon, and when the system is in the 1-photon state the field is necessarily in the vacuum. It will be useful to break the possible states of a system/field pair into three kinds. Since the field is in a superposition of states from which the system will obtain a single photon, each at a different time, it is useful to break the states into those in which the system has not yet absorbed a photon, and refer to the field part of these states as the input field, those in which the system has been promoted to the excited state, and for which the field is thus in the vacuum state, and those for which the system has released its photon back into a field bin, for which the field state will be called the emitted field. 

The Hamiltonian (in the interaction picture) has a very simple form. Since the system interacts with a different bin at each time, it is perhaps simplest if we think of there being a different Hamiltonian acting at each time, $H_j$. The $j^{\mbox{\msi{th}}}$ Hamiltonian is very simple, since it merely has two terms, one of which swaps a photon from bin $j$ to the system and one that swaps a photon from the system to bin $j$. If in the current branch of Hilbert space the bin has a photon and the system does not, the field is converted to the vacuum and the system gains photon. If the system has photon then the photon is transferred to bin $j$ producing a contribution to the single-photon amplitude of the output field. The Hamiltonian is 
\begin{align}
     \hat{H}_j = i\hbar \sqrt{\frac{\gamma}{\Delta t}} \Big( \hat{a}_{\!X}^\dagger \hat{b}_{\!X}(j) - \hat{a}_{\!X}\hat{b}_{\!X}^\dagger(j) \Big)
\end{align}
where $a^\dagger_{\!X}$ is our notation for what ever operator transforms the ground state of the system to the ``one photon" state. Of course the important operator for our purposes is the unitary operator $U_j$ that acts on the system at each time, and all terms in this unitary that are first-order or lower will contribute to the evolution as $\Delta t \rightarrow 0$. 

Let us denote the state of the input field with a photon in bin $j$ by $|1_j\rangle$ and the vacuum by $|\emptyset\rangle$. We will denote the ground state of the mode by $|0\rangle$ and the excited state by $|1\rangle$. The emitted field states (that is, a sate of the field that is a result of a photon being emitted by the mode) we will denote by putting a bar on top: $|\overline{1_j}\rangle$. Note that writing $|1\rangle |\emptyset\rangle$ is actually redundant because the excited state of the system is always accompanied by the vacuum state of the field, so we can write merely $|1\rangle$ as shorthand for this state. 

We will not break the field explicitly into input and output fields. At time-step $j$ the input field is simply all those states with a photon in time bins with index greater than $k$, and the output field is simply all those field states in which the system is in the ground state and the field has a photon in a time bin with index less than $j$. (In the present case the presence of a photon in the field automatically implies that the mode is in the ground state, but for multi-photon inputs this will not always be true.) 

Keeping only terms up to first order in $\Delta t$, the unitary operator is   
\begin{align} 
   U_j =  \hat{\mathbb{I}} \plus \sqrt{\gamma\Delta t} \Big(\hat{a}_{\!X}^\dagger \hat{b}_{\!X}(j) \minus \hat{a}_{\!X}\hat{b}_{\!X}^\dagger(j) \Big) - \frac{\gamma_{\!X}}{2} \Delta t |1\rangle \langle 1 |. 
\end{align}
A key feature of this unitary that is worth noting is the presence of the identity on the right hand side. This, combined with the fact that each bin of the field is acted on only once during the evolution means that any field state that is generated along with the ground state of the system will remain in existence for all time. Another way to say this is that states that are created by $U_j$ will remain for all time unless they contain an excited state of the system, and are thus effected by the final term $-\gamma |1\rangle \langle 1|$. 

Now we have the unitary we can determine how the system and field evolve.  
We can write the initial state of a single system and input field as 
\begin{align} 
   |\psi_0\rangle = \ket{0}\!\sum_{i=1}^\infty \xi_{A}(j) \sqrt{\Delta t} \ket{1_i}
\end{align}
Thus all field states that contain a single photon (that is, have one occupied bin) contain a factor of $\sqrt{\Delta t}$. Thus when we write such a field state we will always group terms in an expression so that the field state contains this factor. 

Now we act with $U_j$ for $j = 1, 2, \ldots$. The identity merely passes the current state through. The second term acts only if the field state is $|\mathbf{1_j}\rangle$ and transforms 
\begin{align} 
    \xi_{A}(j) \sqrt{\Delta t} \ket{0} \ket{1_i} \rightarrow \Delta t \sqrt{\gamma_{\!X}} \xi_{A}(j) |1\rangle \ket{\emptyset} 
\end{align}
This term thus adds the amount $\Delta t \sqrt{\gamma_{\!X}} \xi_{A}(j)$ to the amplitude of the state $|1\rangle \ket{\emptyset}$ at the $j^{\msi{th}}$ time step. 

The third term acts only if the state of the system is excited. If the current amplitude of the excited state is $\psi_1$ then at time $j$ this term produces 
\begin{align} 
   \psi_{1} |1\rangle\ket{\emptyset} \rightarrow  - \sqrt{\Delta t \gamma_{\!X}} \psi_1 \ket{0} \ket{1_j} 
\end{align} 
Since this bin will no longer interact with the system, this emitted field is now preserved, and the output field thus contains a field state with the amplitude $-\sqrt{\gamma} \psi_1(t)$ at time $t$. Thus the emitted field amplitude is $-\sqrt{\gamma} \psi_1(t)$.  The output field (all the field states in which the system is left in the ground state) is thus given by 
\begin{align} 
- \sqrt{\gamma} \psi_1(t) + \xi_{A}(t). 
\end{align} 

We can now put the above facts together to derive the equation of motion for the system. If at time $k-1$ the state of the system and field is given by 
\begin{align} 
   |\psi_{k\!-\!1}\rangle =  \ket{0}\!\sum_{i=1}^\infty \xi_{A}(j) \sqrt{\Delta t} \ket{1_i} + \psi_1(k\!-\!1) \ket{1}\ket{\emptyset} + |0\rangle \left( \sqrt{\Delta t \gamma} \sum_{j=1}^{k-1} f(j) \ket{\overline{1_j}} \right)
\end{align} 
Then applying $U_k$ we have 
\begin{align} 
   |\psi_k\rangle = |\psi_{k\!-\!1}\rangle + \Delta t \left[ \sqrt{\gamma_{\!X}} \xi_{A}(k) -  \frac{\gamma_{\!X}}{2} \psi_1(k-1) \right] |1\rangle\ket{\emptyset} + |0\rangle \left( \sqrt{\Delta t\gamma_{\!X}} \psi_1(k)  \ket{\overline{1_k}} \right)
\end{align} 
giving us immediately the update rule 
\begin{align} 
   \psi_1(k) & =  \psi_1(k\!-\!1) + \Delta t \left[ \sqrt{\gamma_{\!X}} \xi_{A}(k) -  \frac{\gamma_{\!X}}{2} \psi_1(k\!-\!1)  \right] 
\end{align}
or 
\begin{align} 
   \dot\psi_1 & =  -  \frac{\gamma}{2} \psi_1(t) + \sqrt{\gamma_{\!X}} \xi_{A}(t) 
\end{align}n
and the io-relation 
\begin{align} 
  \alpha_{\ms{out}} = \xi_{A}(t)  - \sqrt{\gamma_{\!X}} \psi_1(t) . 
\end{align}
We have now derived the equations of motion of a system interacting with a single io-channel with a single photon input. 

\subsubsection{Two modes, each with (mutually independent) single-photon inputs}

We are now going to show how to derive the joint output field when there are two output channels and the system (now consisting of two cavities, one coupled to each field) emits a photon into each one. Very similar is the situation in which there is a single output field and the system emits two photons into it. The reason these are so similar is because in the limit as $\Delta t \rightarrow 0$ there is essentially no probability that the two output photons can be in the same bin, and the two photons may as well be in different output channels. 

Our two cavities will not be exchanging photons, but could become entangled, for example, via a cross-Kerr interaction that generates an additional phase shift if and only if the is a photon in both cavities. 

The unitary in this case is 
\begin{align} 
   U_j = \hat{\mathbb{I}} \plus \sqrt{\gamma\Delta t} \Big(\hat{a}_{\!X}^\dagger \hat{b}_{\!X}(j) \minus \hat{a}_{\!X}\hat{b}_{\!X}^\dagger(j) + \hat{c}_{\!X}^\dagger \hat{d}_{\!X}(j) \minus \hat{c}_{\!X}\hat{d}_{\!X}^\dagger(j) \Big) - \frac{\gamma}{2} \Delta t \left(|10\rangle \langle 10 | + |01\rangle \langle 01 | + 2 |11\rangle \langle 11|\right). 
\end{align} 
here we have now dropped the subscript ``$X$'' from the decay rate $\gamma$ to make the notation more compact. 

If the two systems are completely independent, then the total envelope for the output fields will be merely the product of that for each field (since this is the tensor product of the states of the output fields). If we denote the excited-state amplitudes for systems A and B by $\psi_{\ms{A}}$ and $\psi_{\ms{B}}$, and the input single-photon envelopes by $\xi_{A}(t)$ and $\xi_{B}(t)$, then the total output two-photon envelope is 
\begin{align}
   \alpha_{\ms{out}}(t,t') = \left[ \xi_{\ms{A}}(t) - \sqrt{\gamma}\psi_{\ms{A}}(t) \right] \left[\xi_{\ms{B}}(t) - \sqrt{\gamma}\psi_{\ms{B}}(t)\right] . 
\end{align} 

The key to determining the output envelope when the two systems are interacting is to note that an output from both cavities can be generated in two distinct ways. One is when the first cavity absorbs a photon and emits it before the other one does so, so that there is no time at which both cavities are excited. The second is a path in which both cavities are excited for some period of time. 

The two-time output amplitude that involves two emissions, the first from cavity 2 and the second from cavity 1, can be written in terms of conditional amplitudes as 
\begin{align}
  \alpha_2(t,t') = \gamma  \psi_{10}(t'| 10,t) \psi_{01}(t) +  \gamma \psi_{10}(t'| 11,t) \psi_{11}(t) 
\end{align} 
Here $\psi_{01}(t)$ is the amplitude that cavity 2 is excited at time $t$ (and thus emits a photon at time $t$), and $\psi_{10}(t'| 10,t)$ is the conditional amplitude that cavity 1 is excited at time $t'$ when cavity 2 was excited at time $t$. The evolution of $\psi_{10}(t'| 10,t)$ is given by the evolution of $\psi_{10}$, but it starts at $0$ at time $t$, and is driven by the input field from that time, because it exists in the subspace in which cavity one has not yet absorbed a photon. 

In the above expression, $\psi_{11}(t)$ is the amplitude that both cavities are excited at time $t$ (and thus that cavity 2 emits at that time (as well as being the amplitude that cavity 1 emits at that time)), and $\psi_{10}(t'| 11,t)$ is the conditional amplitude that cavity 1 is excited at time $t'$ given that both cavities were excited at time $t$. The evolution of $\psi_{10}(t'| 11,t)$ is given by that of $\psi_{10}$, but it starts at unity at time $t$, since the cavity is excited, and is no longer driven by the input, since it exists in a subspace in which the cavity has already absorbed a photon. 

To see in more detail how a two-photon sequence is generated, lets look at the case in which there is a period of time in which both cavities are excited. In each time-step $j$ the evolution terms $-\sqrt{\gamma\Delta t} \hat{a}_{\!X}\hat{b}_{\!X}^\dagger(j)$ and $-\sqrt{\gamma\Delta t} \hat{c}_{\!X}\hat{d}_{\!X}^\dagger(j)$ create an emitted field state with a photon at time $j$ (in output fields A and B, respectively) from the available system states. If we denote the four states of the two modes by $|00\rangle, |01\rangle, |10\rangle, |11\rangle$, (we define the state $|10\rangle$ as that with an excitation in mode A) then the one-excitation states $|10\rangle$ and $|01\rangle$ produce photons in the outputs A and B respectively at each time-step, and these are uncorrelated. The two-excitation state, however, when it is acted on by $-\sqrt{\gamma\Delta t} \hat{a}_{\!X} \hat{b}_{\!X}^\dagger(j)$, generates an output photon in field A and the state $|01\rangle$ which can then be acted on by $-\sqrt{\gamma\Delta t} \hat{c}_{\!X}\hat{d}_{\!X}^\dagger(j)$ at a later time to generate a correlated photon in output B. We can obtain the joint output envelope in the following way. Let us denote the amplitude of the state $|11\rangle|\ket{\emptyset\emptyset}$ at time $j$ by $\psi_{11}$. This state can decay twice. If mode A emits first at time $j$ this produces the state 
\begin{align} 
   \sqrt{\gamma} \psi_{11}(j) \sqrt{\Delta t} |0 1\rangle |\overline{1_j}\emptyset\rangle 
   \label{frag1}
\end{align}
Once this state has been created its amplitude continues to evolve until it emits its second photon. Note, however, that its amplitude evolves in the subspace in which the system has a vacuum input in both ports. This is because in this subspace the input photons have already been absorbed. So we need to determine the equations of motion that describe the state $|0 1\rangle$ when the input fields are in the vacuum state. Let us call the amplitude of this state $\psi_{01}^{\ms{(o)}}$, where the ``o'' indicates that the state is on the ``output side'' of the dynamics (no incoming photons left to absorb). Since the evolution is Markovian, we can solve for the evolution of this amplitude once, where we set its initial value to $1$, and then this gives us the evolution for any initial value $\psi_{11}(j)$ just by muliplying by $\psi_{11}(j)$ (because the evolution is linear). Note however, that if the evolution of $\psi_{01}^{\ms{(o)}}$ is time-dependent, as is the case below in Mikkel's loading scheme, then we must solve separate evolutions for every initial time $j$. We will denote the evolution of $\psi_{01}^{\ms{(o)}}$ with the initial condition $\psi_{01}^{\ms{(o)}}(0) = 1$, and in which there is no driving field, by $\tilde{\psi}_{01}^{\ms{(o)}}(\tau)$. 

Now, the state in Eq.(\ref{frag1}) produces an amplitude for an output photon at every time-step, where the state generated is 
\begin{align}
  \gamma \Delta t  \tilde{\psi}_{01}^{\ms{(o)}}(j\!+\!k)\psi_{11}(j)  |0 0\rangle |\overline{1_j}\overline{1_{j\!+\!k}}\rangle 
\end{align} 
Thus the contribution to the amplitude for the output fields generated from this double decay process is $\gamma \tilde{\psi}_{01}^{\ms{(o)}}(\!j+\!k)\psi_{11}(j)$ for the output state $|\overline{1_j}\overline{1_{j\!+\!k}}\rangle$. 

The equivalent double-decay process happens also in the reverse order, in which cavity B, decays first at time $j$ and subsequently cavity A decays at $j+k$, producing the final output contribution  
\begin{align}
   \gamma \Delta t  \tilde{\psi}_{10}^{\ms{(o)}}(j\!+\!k)\psi_{11}(j)  |0 0\rangle |\overline{1_{j\!+\!k}}\overline{1_j}\rangle 
\end{align} 
As discussed above, we also have a two-photon output process in which one cavity decays before the other cavity absorbs a photon. If we denote the amplitude that evolves with initial condition at time $t$ equal to zero, and that is driven by the input field only from time $t$ onward by $\tilde{\psi}_{01}^{\ms{(i)}}(\tau)$, then the contribution to the total output field is 
\begin{align}
   \gamma \Delta t  \tilde{\psi}_{01}^{\ms{(i)}}(j+k)\psi_{10}(j)  |0 0\rangle |\overline{1_j}\overline{1_{j\!+\!k}}\rangle 
\end{align}

We can now put together the total output envelope, which is  
\begin{align}
   \alpha(t,t') & = \xi_{\ms{A}}(t) \xi_{\ms{B}}(t') - \sqrt{\gamma}\psi_{10}^{\ms{in}}(t) \xi_{\ms{B}}(t')  -  \sqrt{\gamma}\psi_{01}^{\ms{in}}(t') \xi_{\ms{A}}(t) + \gamma \tilde{\psi}_{01}^{\ms{(o)}}(t'-t)\psi_{11}(t) + \gamma \tilde{\psi}_{01}^{\ms{(i)}}(t'-t)\psi_{10}(t), \;\;\;\; t' > t ,  \label{output1} \\ 
   \alpha(t,t') & = \xi_{\ms{A}}(t) \xi_{\ms{B}}(t') -  \sqrt{\gamma}\psi_{10}^{\ms{in}}(t) \xi_{\ms{B}}(t')  -  \sqrt{\gamma}\psi_{01}^{\ms{in}}(t') \xi_{\ms{A}}(t) + \gamma \tilde{\psi}_{10}^{\ms{(o)}}(t-t')\psi_{11}(t') + \gamma \tilde{\psi}_{10}^{\ms{(i)}}(t-t')\psi_{01}(t') , \;\;\, t > t'  .  \label{output2}
\end{align} 
Here we are denoting the amplitudes of the states $|01\rangle$ and $|10\rangle$ in which there is still a photon in one of the input fields by $\psi_{01}^{\ms{in}}$ and $\psi_{10}^{\ms{in}}$. So to obtain the joint output field we need the equations of motion that give the evolution of $\psi_{11}$, $\psi_{10}^{\ms{in}}$ and $\psi_{01}^{\ms{in}}$,  $\tilde{\psi}_{10}^{\ms{(o)}}$ and $\tilde{\psi}_{01}^{\ms{(o)}}$, and $\tilde{\psi}_{10}^{\ms{(i)}}$ and $\tilde{\psi}_{01}^{\ms{(i)}}$. 

The equations of motion that give the evolution of $\psi_{11}$ are 
\begin{align}
   \dot\psi_{10}^{\ms{in}}  &  =  -\frac{\gamma}{2} \psi_{10}^{\ms{in}} + \sqrt{\gamma} \xi_{\ms{A}}(t)   \\ 
   \dot\psi_{01}^{\ms{in}}  &  =  -\frac{\gamma}{2} \psi_{01}^{\ms{in}} + \sqrt{\gamma} \xi_{\ms{B}}(t)  \\ 
   \dot\psi_{11}  &  =  -\gamma \psi_{11} -i \mu + \sqrt{\gamma} [ \xi_{\ms{B}}(t) \psi_{10}^{\ms{in}} + \xi_{\ms{A}}(t) \psi_{01}^{\ms{in}} ] .
   \label{bothcav0}
\end{align}
The equation of motion for $\tilde{\psi}_{10}^{\ms{(o)}}$ and $\tilde{\psi}_{01}^{\ms{(o)}}$ are 
\begin{align}
   \dot{\tilde{\psi}}_{10}^{\ms{(o)}}(\tau)  &  =  -\frac{\gamma}{2} \tilde{\psi}_{10}^{\ms{(o)}}(\tau), \;\;\; \tilde{\psi}_{10}^{\ms{(o)}}(0) = 1 \\
   \dot{\tilde{\psi}}_{01}^{\ms{(o)}}(\tau)  &  =  -\frac{\gamma}{2} \tilde{\psi}_{01}^{\ms{(o)}}(\tau), \;\;\; \tilde{\psi}_{01}^{\ms{(o)}}(0) = 1 
\end{align}
and those for $\tilde{\psi}_{10}^{\ms{(i)}}$ and $\tilde{\psi}_{01}^{\ms{(i)}}$ are 
\begin{align}
   \dot{\tilde{\psi}}_{10}^{\ms{(i)}}(\tau)  &  =  -\frac{\gamma}{2} \tilde{\psi}_{10}^{\ms{(i)}}(\tau) + \sqrt{\gamma}\xi_{\ms{A}}(\tau+t), \;\;\; \tilde{\psi}_{10}^{\ms{(i)}}(0) = 0 \\
   \dot{\tilde{\psi}}_{01}^{\ms{(i)}}(\tau)  &  =  -\frac{\gamma}{2} \tilde{\psi}_{01}^{\ms{(i)}}(\tau) + \sqrt{\gamma}\xi_{\ms{B}}(\tau+t), \;\;\; \tilde{\psi}_{01}^{\ms{(i)}}(0) = 0 . 
\end{align} 

\vspace{2ex} 

\subsection{Extending to the full gate: two modes, each  loaded by its own auxiliary io-mode} 

We again have two input/output cavities, but now each one is referred to as an ``auxiliary'' and is used to load another ``primary'' cavity with the single photon input. We will refer to each pair of cavities (consiting of a primary cavity and the auxiliary that loads it) as one ``side'' of the combined system, and label them as A and B.

\textbf{Subscript notation:} two subscripts to denote the states of the four cavities. The left subscript refers to side A, and the right to side B. The values are: 0, no photons in either cavity, 1, one photon in the auxiliary cavity, c, one photon in the primary cavity. The equations of the four cavity system are  
\begin{subequations}
\begin{align}
   \dot\psi_{10}  &  = [-\frac{\gamma}{2} - i2\mu|\kappa_{A}(t)| ] \psi_{10}  - i\mu\kappa_{A}^*(t)\psi_{\ms{c}0} + \sqrt{\gamma} \xi_{\ms{A}}(t)   \\
   \dot\psi_{\ms{c}0}  &  = - i2\mu|\kappa_{A}(t)| \psi_{\ms{c}0}  -i\mu\kappa_{A}(t)\psi_{10} \\
   & \nonumber  \\
   \dot\psi_{01}  &  =  [-\frac{\gamma}{2} - i2\mu|\kappa_{B}(t)| ] \psi_{01} -i\mu\kappa_{B}^*(t)\psi_{0\ms{c}}  + \sqrt{\gamma} \xi_{\ms{B}}(t)    \\
   \dot\psi_{0\ms{c}}  &  = - i2\mu|\kappa_{B}(t)| \psi_{0\ms{c}} -i\mu\kappa_{B}(t)\psi_{01} \\ 
   & \nonumber  \\
   \dot\psi_{11}  &  =  [ - \gamma - i2\mu(|\kappa_{A}(t)|+|\kappa_{B}(t)|) ] \psi_{11} - i\mu\kappa_{A}^*(t)\psi_{\ms{c}1} - i\mu\kappa_{B}^*(t)\psi_{1\ms{c}}  + \sqrt{\gamma} [ \xi_{\ms{B}}(t) \psi_{10} + \xi_{\ms{A}}(t)  \psi_{01} ] \\ 
   \dot\psi_{1\ms{c}}  &  =  [ -\frac{\gamma}{2} - i2\mu(|\kappa_{A}(t)|+|\kappa_{B}(t)|) ] \psi_{1\ms{c}} - i\mu\kappa_{A}^*(t)\psi_{\ms{cc}} - i\mu\kappa_{B}(t)\psi_{11} + \sqrt{\gamma} \xi_{\ms{A}}(t)  \psi_{0\ms{c}} \\
   \dot\psi_{\ms{c}1}  &  =  [ -\frac{\gamma}{2} - i2\mu(|\kappa_{A}(t)|+|\kappa_{B}(t)|) ] \psi_{\ms{c}1} - i\mu\kappa_{A}(t)\psi_{11} - i\mu\kappa_{B}^*(t)\psi_{\ms{cc}} + \sqrt{\gamma} \xi_{\ms{B}}(t) \psi_{\ms{c}0} \\
   & \nonumber \\ 
   \dot\psi_{\ms{\ms{cc}}}  &  = [ - i \mu - i2\mu(|\kappa_{A}(t)|+|\kappa_{B}(t)|) ] \psi_{\ms{\ms{cc}}} - i\mu\kappa_{A}(t)\psi_{1\ms{c}} - i\mu\kappa_{B}(t)\psi_{\ms{c}1}  
   \label{bothcav}
\end{align} 
\end{subequations}
The two-photon pathways are 
\begin{align}
  \psi_{11} & \rightarrow L_{01}^{(1)}, L_{0c}^{(1)}  \;\;\;\;\; \mbox{then} \;\;\;\;\; L_{01}^{(1)} \rightarrow   \\ 
  & \nonumber \\ 
  \psi_{11} & \rightarrow L_{10}^{(1)}, L_{\ms{c}0}^{(1)}  \;\;\;\;\; \mbox{then} \;\;\;\;\; L_{10}^{(1)} \rightarrow  \\ 
  & \nonumber  \\ 
  \psi_{1\ms{c}} & \rightarrow  L_{0c}^{(2)}, L_{01}^{(2)} \;\;\;\;\; \mbox{then} \;\;\;\;\; L_{01}^{(2)} \rightarrow  \\ 
  & \nonumber  \\
  \psi_{\ms{c}1} & \rightarrow  L_{\ms{c}0}^{(2)}, L_{10}^{(2)} \;\;\;\;\; \mbox{then} \;\;\;\;\; L_{10}^{(2)} \rightarrow \\
    & \nonumber  \\
  \psi_{10} & \rightarrow  \tilde{\psi}^{(i)}_{01}, \tilde{\psi}^{(i)}_{0c} \;\;\;\;\; \mbox{then} \;\;\;\;\; \tilde{\psi}^{(i)}_{01} \rightarrow \\
  & \nonumber  \\
  \psi_{01} & \rightarrow  \tilde{\psi}^{(i)}_{10}, \tilde{\psi}^{(i)}_{c0} \;\;\;\;\; \mbox{then} \;\;\;\;\; \tilde{\psi}^{(i)}_{10} \rightarrow \\
\end{align} 
Where we have denoted the amplitudes for the states that result from the first emission of a two-photon sequence by ``L'' for ``landing states''. The uncorrelated one-photon emissions are 
\begin{align}
  \psi_{10} & \rightarrow    \\ 
  \psi_{01} & \rightarrow   
\end{align}

The equations of motion for the 4 sets of ``intermediate states'' are 
\begin{subequations}
\begin{align}
   \dot L_{01}^{(1)}  &  = [ -\frac{\gamma}{2} -i 4 B (\tau+t) ] L_{01}^{(1)}  - iB(\tau+t) e^{-i\theta} L_{0c}^{(1)} ,  & L_{01}^{(1)}(0) = 1  \\
   \dot L_{0c}^{(1)}  &  = -i 4 B(\tau+t) L_{0c}^{(1)}  -iB(\tau+t) e^{i\theta} L_{01}^{(1)} ,                                    & L_{0c}^{(1)}(0) = 0  \\ 
   & \nonumber \\
   \dot L_{10}^{(1)}  &  = [ -\frac{\gamma}{2} -i4 A(\tau+t) ] L_{10}^{(1)}  - iA(\tau+t) e^{-i\phi} L_{\ms{c}0}^{(1)} ,    & L_{10}^{(1)}(0) = 1  \\
   \dot L_{\ms{c}0}^{(1)}  &  = -i4 A(\tau+t) L_{\ms{c}0}^{(1)} -iA(\tau+t) e^{i\phi} L_{10}^{(1)} ,                                      & L_{\ms{c}0}^{(1)}(0) = 0 \\
   & \nonumber \\
   \dot L_{01}^{(2)}  &  = [ -\frac{\gamma}{2} -i 4 B(\tau+t) ]L_{01}^{(2)}  - iB(\tau+t) e^{-i\theta} L_{0c}^{(2)} ,  & L_{01}^{(2)}(0) = 0  \\
   \dot L_{0c}^{(2)}  &  = -i 4 B(\tau+t) L_{0c}^{(2)} -iB(\tau+t) e^{i\theta} L_{01}^{(2)} ,                                    & L_{0c}^{(2)}(0) = 1  \\ 
   & \nonumber \\
   \dot L_{10}^{(2)}  &  = [ -\frac{\gamma}{2} -i 4 A(\tau+t) ] L_{10}^{(2)}  - iA(\tau+t) e^{-i\phi} L_{\ms{c}0}^{(2)} ,    & L_{10}^{(2)}(0) = 0  \\
   \dot L_{\ms{c}0}^{(2)}  &  = -i4 A(\tau+t) L_{\ms{c}0}^{(2)} -iA(\tau+t) e^{i\phi} L_{10}^{(2)} ,                                      & L_{\ms{c}0}^{(2)}(0) = 1 \\
   & \nonumber \\
   \dot \psi_{01}^{(i)}  &  = [ -\frac{\gamma}{2} -i 4 B(\tau+t) ]\psi_{01}^{(i)}   - iB(\tau+t) e^{-i\theta} \psi_{0c}^{(i)} + \sqrt{\gamma} \xi_{\ms{A}}(\tau+t),  & \psi_{01}^{(i)}(0) = 0  \\
   \dot \psi_{0c}^{(i)}  &  = -i 4 B(\tau+t) \psi_{0c}^{(i)} -iB(\tau+t) e^{i\theta} \psi_{01}^{(i)} ,                                    & \psi_{0c}^{(i)}(0) = 0  \\ 
   & \nonumber \\
   \dot \psi_{10}^{(i)}   &  = [ -\frac{\gamma}{2} -i 4 A(\tau+t) ] \psi_{10}^{(i)}  - iA(\tau+t) e^{-i\phi} \psi_{c0}^{(i)} + \sqrt{\gamma} \xi_{\ms{B}}(\tau+t),    & \psi_{10}^{(i)}(0) = 0  \\
   \dot \psi_{c0}^{(i)}  &  = -i4 A(\tau+t) \psi_{c0}^{(i)} -iA(\tau+t) e^{i\phi} \psi_{10}^{(i)} ,                                      & \psi_{c0}^{(i)}(0) = 0 
\end{align}
\end{subequations}
Note that sets 3 and 4 are identical respectively to sets 1 and 2 except for the initial conditions. 
The output two-photon envelope is 
\begin{align}
  \mathcal{E}(t,t+\tau) &  = \xi_{A}(t) \xi_{B}(t+\tau) - \sqrt{\gamma}\psi_{10}(t) \xi_{B}(t+\tau)  -  \sqrt{\gamma} \psi_{01}(t+\tau) \xi_{A}(t) \nn \\
  & + \gamma L_{01}^{\ms{(1)}}(\tau)\psi_{11}(t) + \gamma L_{01}^{\ms{(2)}}(\tau)\psi_{1\ms{c}}(t) + \gamma \psi_{01}^{(i)}(\tau)\psi_{10}(t) , \;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\; \tau > 0  \\
    \mathcal{E}(t,t+\tau) &  = \xi_{A}(t-\tau) \xi_{B}(t) - \sqrt{\gamma}\psi_{10}(t-\tau) \xi_{B}(\tau)  -  \sqrt{\gamma} \psi_{01}(\tau) \xi_{A}(t-\tau) \nn \\
  &  + \gamma L_{10}^{\ms{(1)}}(\tau)\psi_{11}(t-\tau) + \gamma L_{10}^{\ms{(2)}}(\tau)\psi_{\ms{c}1}(t-\tau) + \gamma \psi_{10}^{(i)}(\tau)\psi_{01}(t-\tau), \;\;  \tau < 0 .
\end{align} 

\vspace{2ex}

\subsubsection{Examining the output via a direct derivation }

The way to derive the equations of motion above using a ``direct'' approach is to write down the general state of two cavities and two unidirectional fields, and then apply the unitary operator once, which will immediately show how the amplitudes for the various states evolve upon rearranging the resulting terms. However, given the shear number of states this is a laborious process. Nevertheless, we now write down the general form of the state of the joint system, and use it to examine the form of the output field.   

We now break the input field into two independent fields (pre-interaction and post-interaction) and also break the output field explicitly into the input field and the field emitted from the systems. We will denote the amplitudes of the emitted field by $E(\cdots)$. 
% 
\begin{align}
   \ket{\Psi(k)} = 
   &\ket{00} \Bigg[\sum_{i,j=1}^{k-1} \! E(i,j) \ket{\overline{1_i} \overline{1_j}} +  \sum_{i,j=1}^{k-1} \! \xi_{A}(i)\xi_{B}(j)  \ket{1_i 1_j} + \sum_{i,j=1}^{k-1} \! E_A(i) \xi_{B}(j) \ket{\overline{1_i} 1_j} +  \sum_{i,j=1}^{k-1} \! \xi_{A}(i) E_B(j) \ket{1_i \overline{1_j}} \Bigg] \Delta t  ~+ \nn\\
   & \ket{00} \sum_{i,j=k}^\infty \! \xi_{A}(i)\xi_{B}(j)  \ket{1_i 1_j} \Delta t ~+ \nn\\
   &\ket{00}\Bigg[\sum_{i=1}^{k-1}\sum_{j=k}^{\infty} \! E_A(i) \xi_{B}(j) \ket{\overline{1_i} 1_j} +  \sum_{i=k}^{\infty}\sum_{j=1}^{k-1} \! \xi_{A}(i) E_B(j) \ket{1_i \overline{1_j}}  \Bigg] \Delta t ~+\nn\\ 
   &\ket{10} \Bigg[  \sum_{j=1}^{k-1}\overline{\psi}_{10}^{(j)}(k) \sqrt{\gamma_{\!X}} \ket{\emptyset \overline{1_j}} +  \sum_{j=1}^{k-1}\psi_{10}^{(j)}(k) \xi_{B}(j) \ket{\emptyset 1_j} +  \sum_{j=k}^{\infty}\!\psi_{10}^{(j)}(k) \xi_{B}(j) \ket{\emptyset 1_j}\Bigg] \sqrt{\Delta t} ~+\nn\\
   &\ket{01} \Bigg[ \sum_{i=1}^{k-1} \overline{\psi}_{01}^{(i)}(k) \sqrt{\gamma_{\!X}}\ket{\overline{1_i} \emptyset} +  \sum_{i=1}^{k-1} \psi_{01}^{(i)}(k) \xi_{A}(i) \ket{1_i \emptyset} + \sum_{i=k}^{\infty} \psi_{01}^{(i)}(k) \xi_{A}(i) \ket{1_i \emptyset} \Bigg] \sqrt{\Delta t} ~+ \nn\\
  & \ket{11}  \psi_{11}(k) \ket{\emptyset\emptyset}.
  \label{genform}
\end{align}
%
The output field at the start of time-step $k$ (that is, before the systems have interacted with bins $k$) is everything in which the system has no photons, and everything in the bins up to $k-1$. That is, it is the top line of the above equation. 

Note that the overline denotes states for which one of the systems has already generated an output photon. In terms of the equations of motion of the two cavities, these arise from two distinct sources. One are those paths in which one system has absorbed and emitted a photon before the other one absorbs a photon, so that they do not contain a photon at the same time, and the second are those paths in which they do.  

Going from step $k$ to step $k+1$ involves two things. First, now the output bins are all the bins up to bin $k$, so additional bins become part of the output field, and at the same time, the unitary interacts the system with bins $k$, so that the system outputs photons into bins $k$. 

For now we are just going to calculate the contributions to the output field that are generated at time-step $k$. The only terms in the unitary operator $U(k)$ that generate terms in the output field are 
\begin{align}
    I, \sqrt{\gamma_{\!X} \Delta t} a b^\dagger(k),  \sqrt{\gamma_{\!X} \Delta t} c d^\dagger(k), \gamma_{\!X} \Delta t a c b^\dagger(k) d^\dagger(k) . 
    \label{listops}
\end{align}
So the new terms in the output field generated in time-step $k$ by the Identity are merely the terms in lines 2 and 3 that contain bins $k$: 
\begin{align}
   & \xi_{A}(k)\xi_{B}(k)  \ket{1_k 1_k} + \sum_{i=1}^k \! \xi_{A}(i)\xi_{B}(k)  \ket{1_i 1_k} + \sum_{j=1}^k \! \xi_{A}(k)\xi_{B}(j)  \ket{1_k 1_j} +  \nn\\ 
   & \sum_{i=1}^{k-1} \! E_A(i) \xi_{B}(k) \ket{\overline{1_i} 1_k} +  \sum_{j=1}^{k-1} \! \xi_{A}(k) E_B(j) \ket{1_k \overline{1_j}}
   \label{part1}
\end{align}
These are just the terms that describe the input field propagating, and in that sense are fairly trivial. 

The output that is generated by the system is all terms generated by applying the other three operators in the list (\ref{listops}). 
\begin{align}
    &\ket{00} \Bigg[  \gamma_{\!X} \sum_{j=1}^{k-1}\overline{\psi}_{10}^{(j)}(k)  \ket{\overline{1_k} \overline{1_j}} +  \sqrt{\gamma_{\!X}} \sum_{j=1}^{k-1}\psi_{10}^{(k)}(k) \xi_{B}(j) \ket{\overline{1_k} 1_j} +  \sqrt{\gamma_{\!X}} \sum_{j=k}^{\infty}\!\psi_{10}^{(j)}(k) \xi_{B}(j) \ket{\overline{1_k} 1_j}\Bigg] \Delta t ~+\nn\\ 
    &\ket{00} \Bigg[ \gamma_{\!X} \sum_{i=1}^{k-1} \overline{\psi}_{01}^{(i)}(k) \ket{\overline{1_i} \overline{1_k}} +  \sqrt{\gamma_{\!X}} \sum_{i=1}^{k-1} \psi_{01}^{(i)}(k) \xi_{A}(i) \ket{1_i \overline{1_k}} +  \sqrt{\gamma_{\!X}} \sum_{i=k}^{\infty} \psi_{01}^{(i)}(k) \xi_{A}(i) \ket{1_i \overline{1_k}} \Bigg] \Delta t ~+ \nn\\
  & \ket{00} \gamma_{\!X} \psi_{11}(k) \ket{\overline{1_k}\overline{1_k}} \Delta t 
  \label{part2}
\end{align}
We want to see now how the terms in Expressions (\ref{part1}) and (\ref{part2}) give Eqs.(\ref{output1}) and (\ref{output2}) that we derived above for the output field. First, terms 1,2, and 3 of Expression (\ref{part1}) make up the first term in Eq.(\ref{output1}) (and the first term in Eq.(\ref{output2})), and terms 4 and 5 in Expression (\ref{part1}) and 2, 3, 5, and 6 in Expression (\ref{part2}) make up terms 2 and 3 in Eq.(\ref{output1}) (and Eq.(\ref{output2})). The relationship that needs some explanation is how the remaining terms of Expression (\ref{part2}) make up the last two terms in Eqs.(\ref{output1}) and (\ref{output2}). First, term 1 in Expression (\ref{part2}), in continuous time is 
\begin{align}
    \gamma_{\!X} \overline{\psi}_{10}(t',t) . 
\end{align}
This gives  the total amplitude of an emission from cavity 1 at time $t'$ when there was an emission from cavity 2 at previous time $t$. What the derivation above does not show us explicitly is how this total amplitude is generated in terms of the amplitudes of various states (in particular ) at the earlier time $t$. To determine that we have to use the general form in Eq.(\ref{genform}) derive the equations of motion for the amplitudes. By matching up with the RHS of Eq.(\ref{output1}) we have 
\begin{align}
    \overline{\psi}_{10}(t',t) =  \tilde{\psi}_{01}^{\ms{(i)}}(t'-t)\psi_{10}(t) +  \tilde{\psi}_{01}^{\ms{(o)}}(t'-t)\psi_{11}(t) . 
\end{align} 

